The Estimation of Continual Causal Effect for Dataset Shifting Streams

Causal effect estimation has been widely used in marketing optimization. The framework of an uplift model followed by a constrained optimization algorithm is popular in practice. To enhance performance in the online environment, the framework needs to be improved to address the complexities caused by temporal dataset shift. This paper focuses on capturing the dataset shift from user behavior and domain distribution changing over time. We propose an Incremental Causal Effect with Proxy Knowledge Distillation (ICE-PKD) framework to tackle this challenge. The ICE-PKD framework includes two components: (i) a multi-treatment uplift network that eliminates confounding bias using counterfactual regression; (ii) an incremental training strategy that adapts to the temporal dataset shift by updating with the latest data and protects generalization via replay-based knowledge distillation. We also revisit the uplift modeling metrics and introduce a novel metric for more precise online evaluation in multiple treatment scenarios. Extensive experiments on both simulated and online datasets show that the proposed framework achieves better performance. The ICE-PKD framework has been deployed in the marketing system of Huaxiaozhu, a ride-hailing platform in China.

==> old.tex <==
\section{Introduction}
Causal effect estimation has become a cornerstone of decision-making in marketing optimization \citep{hulland1996use, sun2015causal, liu2023explicit}. In marketing optimization, understanding the causal impact of interventions is essential for optimizing outcomes and informing effective strategies within observational data. Confronted with the challenges of missing counterfactual outcomes and selection bias \citep{vemuri2015causal}, considerable efforts have been made, resulting in promising outcomes, such as sample re-weighting \citep{austin2011introduction, bottou2013counterfactual,zubizarreta2015stable,hassanpour2019counterfactual}, balanced representation \citep{bengio2013representation, shalit2017estimating}, disentangled representation \citep{hassanpour2019counterfactual, wu2022learning} and so on.

Although significant progress has been made, existing methods primarily focus on source-only and stationary observational data, assuming that all observational data are available during the training phase. However, this assumption does not align with real-world conditions \citep{chu2023continual}. In marketing, the data source is dynamic, influenced by marketing campaigns and news events. As a result, dataset shift \citep{nair2019covariate}, including covariate shift \citep{nair2019covariate} and concept drift \citep{kull2014patterns}, is common in marketing. The definitions of covariate shift and concept drift discussed here are as follows:

\textbf{Covariate shift} refers to the situation where the distribution of the covariates changes over time. The relationship between the covariates and the responses (or outcomes) is not our concern.

\textbf{Concept drift} refers to the phenomenon where the relationship between the covariates and the responses (or outcomes) changes over time for each treatment. The distribution of the covariates is not our concern.

Subsequently, the Continual Causal Effect Representation Learning method (CERL) is proposed, making the first attempt to address the problem of continual lifelong causal effect estimation \citep{chu2023continual}. CERL focuses on scenarios involving a single treatment and the presence of covariate shift. Although its effectiveness is demonstrated through experiments, businesses frequently encounter the challenge of multiple treatments and complex phenomena such as concept drift in practical marketing environments, which CERL fails to adequately address.

To overcome these limitations, we propose the Incremental Causal Effect with Proxy Knowledge Distillation (ICE-PKD), a method designed to handle multiple treatments and effectively address the complexities associated with concept drift. ICE-PKD provides a more robust and adaptable approach for causal effect estimation in dynamic marketing settings. Specifically, ICE-PKD is built upon the Disentangled Representations for CounterFactual Regression (DR-CFR) framework \citep{hassanpour2019learning} and draws inspiration from class-incremental methods in computer vision \citep{van2022three, belouadah2021comprehensive}, such as functional regularization \citep{li2017learning} and relay-based techniques \citep{rebuffi2017icarl}. Additionally, we introduce a customized modification to the knowledge distillation process by incorporating insights from the alternative method of PTLoss \citep{zhang2024knowledge}, addressing concept drift more effectively. As a result, ICE-PKD overcomes the limitations of previous methods, and its effectiveness has been validated through extensive experiments.

The main contributions of this paper are as follows: (1) We extend the DR-CFR framework to handle multiple treatments; (2) We propose ICE-PKD, the first method for continual causal effect estimation that accounts for concept drift; (3) We provide a novel approach for constructing causal effect estimation streams, considering both covariate shift and concept drift; (4) We introduce a new evaluation metric for marketing scenarios, namely RAS-AUCC; (5) We systematically establish an evaluation framework for continual causal effect estimation, emphasizing both stability and average improvement.

\section{Problem Statement}

Let \( X \) denote the covariate set, \( Y \) denote the set of binary outcomes, and \( T \) denote the set of treatments containing \( |T| \) types  \(0,1, \cdots,|T|-1 \) .
In continual causal effects estimation, the observational data are collected from \( n_k \) different time periods and the $k$-th dataset contains the data \( \{(x,y,t)|x \in X, y \in Y, t \in T \} \) collected from the $k$-th time period, which contains \( n_k \) units. Let \( X \) denote all covariates, \( Y \) denote the binary outcomes, and \( T \) denote treatments containing \( n_t+1 \) distinct types \(0,1, \cdots,n_t \). In the presence of covariate shift and concept drift, datasets \( \{ D_k \}_{k=1}^{n_k} \) have different distributions with respect to \( X \) and different relationships between \( X \) and \( Y \) for each treatment. Let \( t_i \) denote the treatment assignment for unit \( i \). For multiple treatments, only \( t_i=0 \) is for the control group. The outcome for unit \( i \) is denoted by \( y_i^t \) when treatment \( t \) is applied to unit \( i \). For observational data, only one of the potential outcomes is observed, which is called the factual outcome. In contrast, all the remaining unobserved potential outcomes are called counterfactual outcomes. For each time period (except \( 0 \)), the responses \( \hat{y}_i \) of treatments \( t=0,1,\dots,N_t \) applied on a unit \( i \) are predicted to estimate the expected Individual Treatment Effect (ITE) \( \tau_i^t \) under the treatments \( t=1,2,\dots,n_t \). Specifically, under three standard assumptions \citep{rosenbaum1983central, zhong2022descn}, the estimate of \( \tau_i^t \) can be expressed as follows:

\begin{equation}
    \tau_i^t=\mathbb{E}(y_i^t-y_i^0|x_i)=\mathbb{E}(y_i^t|t,x_i)-\mathbb{E}(y_i^0|t,x_i)
\end{equation}

Here, \( \mathbb{E}[y^{t}|t,x] \) represents the expected predicted response \( \hat{y}_i \) of individual \( x_i \) under treatment \( t \), for \( t=0,1,2,...,n_t\). In scenarios such as marketing campaigns, the outcome \( y_i \in \{0,1\} \) typically indicates whether or not the individual made a purchase, and the predicted response \( y_i^t \in [0,1] \) represents the probability of purchase for the individual.

Our objective is to develop a novel continual causal effect inference framework to accurately estimate the causal effects for incrementally available data \( D_k \) in the presence of distribution shift and concept drift.

\section{Methodology}
As discussed in Section \ref{section:uplift modeling}, most existing methods inadequately capture the dynamics prevalent in many industrial applications. This is particularly evident in online marketing, where data sources are influenced by factors such as news, holidays and weather conditions. Those lead to variations in crowd distribution across different time periods (i.e. covariate shift), while individual behaviors and perceptions evolve continuously (i.e. concept drift). 

To address the above challenges, we propose Incremental Causal Effect with Proxy Knowledge Distillation (ICE-PKD), an efficient method for performing uplift modeling on incrementally available data, even amidst covariate shift and concept drift. The architecture of ICE-PKD is illustrated in Figure \ref{alg:ice-pkd}. Specifically, DRCFR serves as the base model of ICE-PKD, providing robust causal inference capabilities in multi-treatment observational data scenarios. The initial model selection ensures reliable generalization before incremental training. Parameter initialization enhances the efficiency of incremental training by necessitating only a smaller learning rate and fewer training epochs. Knowledge distillation preserves previous knowledge while adapting to new changes. The replay mechanism maintains the accuracy and stability of the knowledge distillation process in the presence of covariate shift. Transforming the original teacher model into a proxy teacher improves both the accuracy and reliability of the knowledge distillation, particularly in the context of concept drift. It ensures that the student model does not blindly imitate the teacher.

\begin{figure}
    \centering
    \includegraphics[height=6cm]{ICE-PKD2.pdf} 
    \caption{The architecture of ICE-PKD}
    \label{fig:ice-pkd}
\end{figure}

\subsection{The Base Causal Effect learning Model}
In this section, we describe the base model for causal effect estimation in observational datasets. This component is equivalent to the traditional causal effect learning problem, serving as the foundation for continual incremental causal effect learning. A key challenge in estimating causal effects from observational data is selection bias, where the distribution of data varies across treatment groups. This issue is particularly pronounced when there are few sample instances within a given domain for each treatment group, complicating precise inferences about counterfactual outcomes.

To address this challenge, we employ the DRCFR framework \citep{hassanpour2019learning}. This framework disentangles covariates into underlying factors and balances the representation of confounders between control and treatment groups. This method is particularly effective in enhancing the accuracy of causal effect estimation. In this paper, we extend it to accommodate multiple treatment scenarios while satisfying the monotonicity condition.

\paragraph{Learning Disentangled Representations.}
We assume that all covariates influencing the effect of the model are generated by three underlying factors $\{ \Gamma,\Delta,\Upsilon \}$ \citep{hassanpour2019learning}. The instrumental factor $\Gamma$ affects only the treatment assignment, the confounding factor $\Delta$ influences both the treatment and the outcome, and the adjustment factor $\Upsilon$ determines only the outcome. While the presence of instrumental and confounding factors introduces selection bias, confounding factors can still provide useful information for accurately estimating the response. To model these factors, we employ three representation learning networks \( \Gamma(x) \), \(\Delta(x) \) and \( \Upsilon(x) \), which learn the respective factors from data.

\paragraph{Re-Weighting Function.}
To address the selection bias in estimating Individual Treatment Effects, \citep{hassanpour2019learning} employs context-aware importance sampling, where the weights are derived exclusively from \(\Delta(x)\). In this work, we extend this approach to accommodate the multi-treatment scenario:
% Given the differences in the distribution of various sample instances, we further reduce the impact of selection bias on the ITE estimation by incorporating contextual information for each instance's learned representation, \(\Delta(x)\) and the weights are computed based solely on \( \Delta(x) \) \citep{hassanpour2019learning}. The distinction here is that we extend DR-CFR to the multi-treatment scenario.
\begin{equation}
    w(t_{i},\Delta(x_{i}))=1+\sum_{j\ne i} \frac{p(t_{i})}{p(t_{j})} \cdot \frac{\pi(t_{j}\mid \Delta(x_{i}))}{\pi(t_{i}\mid \Delta(x_{i}))}
\end{equation}

\paragraph{Imbalance Loss.}
Based on the definition of the adjustment factor \( \Upsilon \), the distribution of learned adjustment factors \( \Upsilon(x) \) should be similar across treatment groups \citep{hassanpour2019learning}. To quantify the distributional differences of \( \Upsilon(x) \), \citet{hassanpour2019learning} utilize the Wasserstein distance, incorporating it as a penalty term in the loss function. We now extend this formulation to the multi-treatment case:  
\begin{equation}
 L_{Im}=\sum_{t=1}^{|T|} disc(\left \{ \Upsilon(x_{i})\right\}_{i:t_{i}=0} ,\left \{ \Upsilon(x_{i})\right\}_{i:t_{i}=t})
\end{equation}

\paragraph{Cross Entropy Loss.}
The combined representations of instrument factors and confounding factors contain sufficient information to reconstruct the decision rules for the treatment assignment \citep{hassanpour2019learning}. Therefore, \citet{hassanpour2019learning} leverage the learned representations $\Gamma(x)$ and $\Delta(x)$ to predict the assigned treatments, minimizing the loss function to ensure that all relevant information pertaining to treatment assignments is captured in these two representations. The following formula defines the loss function in the multi-treatment case:
\begin{equation}
    \pi(t|\Gamma(x),\Delta(x)) =\frac{e^{\varphi(\Gamma(x) ,\Delta(x) ) }_{t}}{\sum_{t=0}^{|T|}e^{\varphi(\Gamma(x) ,\Delta(x) ) }_{t}} 
\end{equation}

\begin{equation}
    L_{CE}=\frac{1}{N}\sum_{i=1}^{N}-\log \left[\pi \left( t_{i}|\Gamma(x_{i}),\Delta(x_{i}) \right) \right]
\end{equation}

\paragraph{Multi-task Learning Architecture for Estimating Factual Loss.}
The combination of the learned representations \( \Delta(x) \) and \( \Upsilon(x) \) retains sufficient information for accurate factual estimation. In scenarios with a finite number of treatments, drawing inspiration from the TarNet framework \citep{shalit2017estimating}, we employ a multi-task learning structure for factual estimation using \( \Delta(x) \) and \( \Upsilon(x) \). Specifically, each treatment \( t \) corresponds to a separate task network \( h^t(\cdot) \). We first obtain a shared representation for all tasks by passing the union of \( \Delta(x) \) and \( \Upsilon(x) \) through a network. Subsequently, each task network \( h^t(\cdot) \) is trained independently, allowing the model to learn treatment-specific responses while sharing common features across tasks. This multi-task approach enhances learning efficiency by leveraging shared information across treatments while capturing the nuances of each treatment assignment. When the outcome \( Y \) is binary, the factual loss function is calculated as follows:
\begin{equation}
    L_{Fac}(x, y, t) = - \left[ y \log \left( h^t(\Delta(x), \Upsilon(x)) \right) + (1 - y) \log \left( 1 - h^t(\Delta(x), \Upsilon(x)) \right) \right]
\end{equation}

\paragraph{ATE Loss.}
In certain business contexts, such as optimizing the ROI for marketing campaigns, the accuracy of the uplift model's predictions is as crucial as the ranking of treatment effects. This underscores the necessity of minimizing the ATE Error. Drawing inspiration from the concept of ATE Error in uplift models, we propose the ATE loss function to reduce the ATE Error and enhance prediction accuracy. Specifically, the ATE loss is defined as the absolute difference between the predicted average treatment effect \( \hat{\text{ATE}}_t \) and true average treatment effect \( \text{ATE}_t \) for each treatment level \( t \):
\begin{equation}
    L_{ATE}=\frac{1}{|T|}\sum_{t=1}^{|T|} |\hat{\text{ATE}}_t - \text{ATE}_t| = \frac{1}{N \cdot |T|}\sum_{t=1}^{|T|} | (\sum_{i=1}^{N}\hat{y}_{i:t_i=t}-\sum_{i=1}^{N}\hat{y}_{i:t_i=0}) - (\sum_{i=1}^{N}y_{i:t_i=t}-\sum_{i=1}^{N}y_{i:t_i=0})|
\end{equation}

\paragraph{Monotonicity Penalty Loss.}
In online scenarios, such as modeling user purchase propensity at varying discount levels, the monotonicity assumption is often regarded as prior knowledge. As the treatment level increases, the individual response is expected to increase. To incorporate this knowledge into our model, we introduce the concept of monotonicity penalty loss, which penalizes any violation of this monotonicity assumption. The loss function is defined as follows:
\begin{equation}    L_{Mono}=\frac{1}{N}\sum_{i=1}^{N}\sum_{t=1}^{|T|}\text{ReLU}(\hat{y}_i^{t-1}-\hat{y}_i^{t})
\end{equation}

Here, \( \text{ReLU} \) denotes the rectified linear unit function, which ensures that the penalty is applied only when the predicted response at the higher treatment level is less than the smaller.

\paragraph{Overall Loss Function of DR-CFR}
In this section, we review the previously introduced loss functions and present the overall loss function for the base causal effect learning model, defined as:
\begin{equation}
\begin{aligned}
L_{Base}&=\frac{1}{N}\sum_{i=1}^{N}w(t_{i},\Delta(x_{i}))\cdot L_{Fac}(x_i,y_i,t_i)\\
&+\alpha \cdot L_{CE} + \beta \cdot L_{Im} + \gamma \cdot L_{ATE} + \delta \cdot L_{Mono} + \lambda \cdot L_{Reg}\\
\end{aligned}
\end{equation}

where \( L_{Reg} \) is the regularization term, \( \alpha \), \( \beta \), \( \gamma \), \( \delta \) and \( \lambda \) are hyperparameters that control the scale of each component.

\subsection{The Continual Incremental Causal Effect Learning}
Building on the base causal effect learning model, we propose the ICE-PKD framework. By first training a well-generalized initial model on the initially available data and then updating it with incrementally available data, this method effectively addresses both covariate shift and concept drift.

\paragraph{Initial Model Selection and Parameter Initialization.}
Due to the complexity of the uplift model, random initialization of the parameters can lead to large perturbations in performance. Therefore, we train the model multiple times on the initially available data and select the optimal model \( g_{\theta_0}^t(x) \). The primary evaluation metric used here is RAS-AUCC, which is introduced in the next chapter. Furthermore, similar to the incremental learning approach \citep{li2017learning,rebuffi2017icarl} in computer vision, we initialize the parameters of the incremental model based on the parameters of the previous incrementally trained model. Specifically, during the $k$-th incremental training of the model, we initialize the model parameters \( \theta_{k} \) with \( \theta_{k-1} \), which are the parameters obtained after the $(k-1)$-th incremental training.

\paragraph{Loss Function Regularization via Knowledge Distillation.}
To ensure the generalization of the model during incremental training, we draw inspiration from the class-incremental method LwF \citep{li2017learning}, which is based on knowledge distillation, from the computer vision domain and apply it to the uplift model scenario. Under the assumption of concept drift, our primary focus is the difference in predicted distributions between the model before and after incremental training, rather than the predicted values themselves. Specifically, we are interested in the discrepancy between the model \(g_{\theta_k}(x) \) and the model \( g_{\theta_{k-1}}(x) \). To quantify this difference, we use the Kullback-Leibler (KL) Divergence. In the context of a binary classification problem, the KL Divergence is computed as:
\begin{equation}
    D_\mathrm{KL}(y\parallel\hat{y})=y\log\frac{y}{\hat{y}}+(1-y)\log\frac{1-y}{1-\hat{y}}    
\end{equation}

where $y$ represents the true label and $\hat{y}$ represents the predicted probability.

Thus, the knowledge distillation loss function $L_{KD}$ during the $k$-th incremental training is defined as:
\begin{equation}
    L_{KD}=\frac{1}{N} \sum_{i=1}^{N} \sum_{t=0}^{|T|} D_\mathrm{KL}(g_{\theta_{k-1}}^{t}(x_i)\parallel{g_{\theta_{k}}^{t
}(x_i)})  
\end{equation}

where the superscript \( t \) represents the response of the model under the treatment \( t \) or without treatment (i.e. \( t = 0 \)), \( \theta_{k-1} \) are the model parameters after the $(k-1)$-th incremental training (which remain fixed during this process), \( \theta_{k} \) are the model parameters to be updated during the current incremental training process.

By penalizing the difference in predictive distributions between the model before and after incremental training, we aim to preserve prior knowledge and mitigate catastrophic forgetting under the assumption of concept drift.

\paragraph{Replay Mechanism.}
Due to the presence of covariate  shift, relying solely on new data to calculate distributional difference for preserving previous knowledge becomes unfeasible, as neural networks tend to perform poorly when predicting out-of-distribution data. Drawing inspiration from the class-incremental method iCaRL \citep{rebuffi2017icarl} in computer vision, we aim to apply knowledge distillation on a replayed subset of the previous dataset. However, unlike image classification tasks, the sample or feature centers do not play a significant role in this scenario. Therefore, we adopt a uniform sampling approach, where approximately one percent of the total initial sample size from the previous dataset is preserved as representation of recent data used for incremental training. Specifically, 
\begin{equation}
    N_{save}=\left\lfloor 0.01 \cdot \tilde{N}_0 \right\rfloor
\end{equation}

where \( \tilde{N}_0 \) is the sample number used for training the base model, and \( N_{save} \) represents the integer part of \( 0.01 \cdot \tilde{N}_0 \).

After the $(k-1)$-th incremental training, we have not only model parameters \( \theta_{k-1} \), but also the replayed dataset \( R_{k-1} \)consisting of \( N_{save} \) samples, and the total number \( \tilde{N}_{k-1} \) of samples used for previous training. During the $k$-th incremental training, the latest available dataset \( D_{k} \) with \( N_{k} \) samples is used. Now, the total number of samples used for training is updated by:
\begin{equation}
    \tilde{N}_{k} = \tilde{N}_{k-1} + N_{k}
\end{equation}

To determine the size of the replayed dataset \( R_{k} \) from  \( R_{k-1} \) and \( D_{k} \), we calculate:
\begin{equation}
    N_{save}^R,N_{save}^D = \lfloor \frac{N_{save} \cdot \tilde{N}_{k-1}}{\tilde{N}_{k}} \rfloor, \lceil \frac{N_{save} \cdot N_{k}}{\tilde{N}_{k}} \rceil
\end{equation}

To perform the uniform sampling, we generate sequences of random numbers:
\begin{equation}
    r_1,r_2,\ldots,r_{N_{save}},d_1,d_2,\dots,d_{N_{k}} \sim U(0,1)
\end{equation}

where \( \{ r_i \}_{i=1}^{N_{save}} \) , \( \{ d_i \}_{i=1}^{N_{k}} \) are sequences of random numbers corresponding to the ordinal numbers of the dataset \( R_k \) and \( D_{k} \). These random sequences are sorted, and
then we take the first \( N_{save}^R \) samples and \( N_{save}^D \) samples together as the replayed dataset \( R_{k} \) for $(k+1)$-th incremental training.

\paragraph{Proxy Teacher for Knowledge Distillation.}
Due to the presence of concept drift, there is a natural discrepancy in the output distributions of the teacher model used for knowledge distillation, even without considering training bias. In this context, it is unwise to force the model to blindly imitate the unreliable teacher model \( g_{\theta_{k-1}}(x) \) during the $(k)$-th incremental training. To this end, we transform the original teacher into a proxy teacher by introducing a corrector \( h_{\theta_c}(x) \) in the calculation of KL divergence, which is inspired by the alternative solution of PTLoss \citep{zhang2024knowledge} and making corresponding modifications. Specifically, the loss function used for knowledge distillation at this point is calculated as follows:
\begin{equation}
    L_{PT}=\frac{1}{N} \sum_{i=1}^{N} \sum_{t=0}^{|T|} D_\mathrm{KL}(g_{\theta_{k-1}}^{t}(x_i)+h_{\theta_c}^{t}(x_i)\parallel{g_{\theta_{k}}^{t}(x_i,t)})  
\end{equation}

which is similar to equation(11). The difference is the addition of a corrector \( h_{\theta_c} \), which is a neural network with the same input covariates and output dimensions as \( g_{\theta_{k-1}}(x) \).

From the perspective of training stability and feasibility, we set the activation function of the hidden layers of \( h_{\theta_c} \) to ReLU, the activation function of the output layer to Tanh, and use the Xavier initialization method to ensure that the output values of the \( h_{\theta_c} \) are small before training. Intuitively, this avoids large perturbations to the teacher model at the beginning of training and allows for more rapid convergence, which is compatible with incremental learning using a smaller learning rate and fewer training epochs.

After making such a modification, in addition to the model's parameter \( \theta_{k} \) updates being subject to the previous knowledge (i.e. teacher model \(g_{\theta_{k-1}}(x)\)), the teacher model is also guided and corrected by the new data during the $(k+1)$-th incremental training. 

\paragraph{Overall Loss Function of ICE-PKD.}
The overall loss function of ICE-PKD during the $k$ -th incremental training is calculated as follows:
\begin{equation}
    L_{ICE-PKD} = L_{Base}|D_{k} + \mu \cdot L_{PT}|R_{k-1}
\end{equation}

where \( \mu \) is a weighting coefficient, \( L_{Base}|D_{k} \) denotes \( L_{Base} \) computed on the latest available dataset \( D_{k} \) and \(  L_{PT}|R_{k-1} \) represents \( L_{PT} \) calculated on the replayed dataset \( R_{k-1} \).

Finally, we summarize the procedures of ICE-PKD. The pseudo code of AutoSurvey can be found at Algorithm \ref{alg:ice-pkd}.
% The algorithmic flow is shown in Algorithm

\begin{algorithm}[H]
\caption{Incremental Causal Effect with Proxy Knowledge Distillation (ICE-PKD)}
\label{alg:ice-pkd}
\begin{algorithmic}[1]
\REQUIRE Initial dataset $D_0$, incremental data sequence $\{D_k\}_{k=1}^{n_k}$
\ENSURE Trained model $\theta_k$ for $k=1,\cdots,n_k$

\STATE \textbf{Initialize:}
\STATE Train base model: $\theta_0 \gets \arg\min_\theta L_{Base}|D_0$
\STATE Initialize replay buffer: $R_0 \gets \text{UniformSample}(D_0, N_{save})$
\STATE Set total sample count: $\tilde{N}_0 \gets N_0$

\FOR{$k=1$ \TO $n_k$}
    % \STATE \textbf{Parameter Initialization:}
    \STATE $\theta_k \gets \theta_{k-1}$ \COMMENT{Inherit previous parameters}
    
    % \STATE \textbf{Proxy Teacher Construction:}
    \STATE Initialize corrector network $h_{\theta_c}$ with Xavier initialization
    \STATE Build proxy teacher: $g_{\theta_{k-1}}^{t}(x) + h_{\theta_c}^{t}(x)$
    
    % \STATE \textbf{Data Preparation:}
    \STATE Merge datasets: $\mathcal{D}_{train} \gets D_k \cup R_{k-1}$
    \STATE Update total samples: $\tilde{N}_k \gets \tilde{N}_{k-1} + N_k$

    % \STATE \textbf{Replay Buffer Update:}
    \STATE Compute sample sizes: 
    \STATE $\quad N_{save}^R \gets \lfloor N_{save} \cdot \tilde{N}_{k-1} /\ \tilde{N}_{k} \rfloor$
    \STATE $\quad N_{save}^D \gets \lceil N_{save} \cdot N_{k} /\ \tilde{N}_{k} \rceil$
    \STATE $R_k \gets \text{UniformSample}(R_{k-1}, N_{save}^R) \cup \text{UniformSample}(D_k, N_{save}^D)$
    
    % \STATE \textbf{Incremental Training:}
    \FOR{epoch $=1$ \TO epochs}
        \STATE Compute base loss: $\mathcal{L}_{base} \gets L_{Base}|D_k$
        \STATE Compute proxy loss: $\mathcal{L}_{pt} \gets  L_{PT}|R_{k-1}$
        \STATE Update parameters: $\theta_k \gets \theta_k - \eta\nabla_{\theta}(\mathcal{L}_{base} + \mu \cdot \mathcal{L}_{pt})$
        \STATE Update corrector: $\theta_c \gets \theta_c - \eta\nabla_{\theta_c}\mathcal{L}_{pt}$
    \ENDFOR
\ENDFOR

\RETURN $\theta_k$ for $k=1,\cdots,n_k$
\end{algorithmic}
\end{algorithm}

\section{Experiments and Evaluations}

\subsection{Description of the datasets}
To accurately assess the model performance, we conduct experiments on synthetic datasets \citep{berrevoets2019causal} that adhere to our assumptions and provide access to a ground truth (i.e., counterfactual outcomes). Additionally, we validate the results using an online dataset to demonstrate the practical applicability and significance of the proposed method. The datasets are described as follows:

\subsubsection{Synthetic Dataset}
We first consider a 2-dimensional synthetic dataset \citep{berrevoets2019causal} with three treatments, which facilitates both analysis and visualization. For each time period \( k \), the exact responses under different treatments are given by the following equations:
\begin{align}
    p_{k,0}(x_1,x_2) &= \sigma\left(0.6x_1^2 + x_1x_2^2 - (0.5-d_0(k))\cdot x_1 - (0.6 - 0.5d_0(k)) \cdot x_2 + 0.2d_0(k) + \epsilon \right) \\
    p_{k,1}(x_1,x_2) &= \sigma\left(0.7x_1^2 + 0.1x_2^2 + x_1x_2^2 - (0.5-d_1(k))\cdot x_1 - (0.5 - 0.5d_1(k)) \cdot x_2 + 0.2d_1(k) + \epsilon \right) \\
    p_{k,2}(x_1,x_2) &= \sigma\left(0.9x_1^2 + 0.15x_2^2 + x_1x_2^2 - (0.5-d_2(k))\cdot x_1 - (0.5 - 0.5d_2(k)) \cdot x_2 + 0.2d_2(k) + \epsilon \right)
\end{align}

where \( x_1,x_2 \in [0,1] \), and \( \sigma( \cdot ) \) represent the logistic sigmoid function, which maps the polynomial expressions to a range of \( [0,1] \). The term \( \epsilon \sim \mathcal{N}(0, 0.0001) \) denotes Gaussian noise, and \( x = (x_1, x_2) \) is a covariate with two components. The treatments \( t=0,1,2 \) correspond to different coupon amounts, while \( d_0(k), d_1(k), d_2(k) \) represent concept drift that varies over time, indexed by the time period \( k \). The specific relationship between \(d_i(k)\) and \( k \) is defined as follows:
\begin{equation}
    d_i(k)=\begin{cases} 
0.1ik + 0.2k & \text{if } 0 \leq k \leq 3 \\
-0.1ik + 0.65i - 0.2k + 1.3 & \text{if } 4 \leq k \leq 6 
\end{cases}
\quad \text{for } i = 0, 1, 2
\end{equation}

\begin{figure}
    \centering
    \includegraphics[height=6cm]{func_0.png} 
    \caption{Response Function Visualization for \(k=0\).}
    \label{fig:fig2}
\end{figure}

The visualization of the response function for time period \( k=0 \) is presented in Figure~\ref{fig:fig2}, where the blue surface represents the response function under \( t=0 \), the red surface corresponds to  \( t=1 \), and the green surface depicts \( t=2 \). As shown in Figure~\ref{fig:fig2}, the generated functional relationship adheres to the monotonicity assumption, which aligns with business expectations. Specifically, this means that the user's willingness to purchase increases as the discount rises. Mathematically, this is expressed as: 
\begin{equation}
    \forall k, \quad p_{k,2}(x_1, x_2) \geq p_{k,1}(x_1, x_2) \geq p_{k,0}(x_1, x_2) \quad \text{a.e.} \ x_1, x_2 \in [0, 1]
\end{equation}

To satisfy the assumption of covariate shift, we generate a training covariate dataset of size 10,000 and a test covariate dataset of size 50,000 from four truncated normal distributions and one uniform distribution for each time period \( k \). The means of the truncated normal distributions are randomly chosen from the range \( [0.2,0.8] \), and their standard deviations are randomly selected from the range \( [0.01,0.1] \), with the covariance set to zero. According to the properties of normal distributions, most of the points lie within the domain \( [0,1] \times [0,1] \), and any points outside this domain are truncated to fall within the domain boundaries. The uniform distribution is denoted as \( U[0,1] \). 

Based on Eq. (19), (20), and (21), we can derive the exact response probabilities under the three treatments, which are then used to evaluate the Precision in Estimation of Heterogeneous Effect (PEHE). Moreover, these response probabilities serve as parameters in Bernoulli experiments to generate the corresponding labels. 

In the test dataset, each covariate is randomly assigned a treatment along with its corresponding label, ensuring no selection bias. For the training dataset, treatments are applied to each covariate according to predefined rules. Specifically, when \( x_1 + x_2 < 0.8\), neither the uplift from \( t=0 \) to \( t=1 \) nor the uplift from \( t=1 \) to \( t=2 \) is significant. In this case, we prefer to apply treatment \( t=0 \) to covariates in this region, while the probabilities of applying \( t=1 \) or \( t=2 \)  are both relatively low. In practice, we perform a Bernoulli test with a probability of 0.6 and apply \( t=0 \) if the result is successful; otherwise, we perform another Bernoulli test with a probability of 0.5 and apply \( t=1 \) if the result is successful. If neither test is successful, we apply \( t=2 \). Similarly, when \( x_1 + x_2 > 1.2 \), treatment \( t=1 \) is preferred, while for \( 0.8 \leq x_1 + x_2 \leq 1.2 \), treatment \( t=2 \) is preferred.

For the 10-dimensional synthetic dataset, we simulate the process used for the 2-dimensional dataset. The primary difference lies in the higher dimensionality, which results in a larger dataset for both training and testing.

\subsubsection{Online Dataset}
In Huaxiaozhu's new passenger acquisition campaign, we have access to sufficient data that exhibits both covariate shift and conceptual drift. To capture these dynamics, we divide the data over time, following the model updating strategy used in previous work. Specifically, the non-incremental model updating strategy utilizes around 1 million records from the past 9 weeks each week, balancing considerations such as resource constraints and model effectiveness. For each time period \( k \), the records from the subsequent week are considered as the test dataset. We use approximately 120,000 new passenger records each week as an incremental training set \( D_k \) for time period \( k=1,2,\cdots,6 \), while the initially available dataset consists of around 1 million records from the 9 weeks prior to the start of the experiment. 

For modeling, we utilize a 53-dimensional feature space, which includes covariates such as city-specific characteristics and historical statistics. The campaign involves eight treatment levels, corresponding to coupon amounts \( 3,4, \dots,10 \), with the treatments indexed as \( t=0,1, \dots, 7 \). The control group is represented by \( t=0 \), corresponding to a minimum coupon amount of \( 3 \). The outcome label \( y \in \{ 0,1 \} \) indicates whether an order is completed (\( y=0 \)) or not (\( y=1 \)). 

\subsection{Experimental Setting}
\label{section:experimental setting}
For the synthetic dataset, we sequentially split the 10\% of each training dataset for time period \( k \) as the available dataset \( D_k \), which leads to a noticeable decrease in online performance over time. To predict the test dataset for each time period \( k \), where \( k=1,2,\cdots,6\), we apply our model, ICE-PKD, along with three comparison strategies. In the incremental updating of \textbf{ICE-PKD}, we begin by selecting an initial model \( g_{\theta_0}^t(x) \), which achieves the best performance on the initially available data (i.e. the entire training dataset at time period \( k=0 \)) and then update the model incrementally with \( D_k \) for each \( k=1,2,\cdots,6 \). To further demonstrate the effectiveness of ICE-PKD, we compare it with three alternative strategies: \textbf{DRCFR A} trains the DR-CFR using the entire training dataset from the previous time period \( k-1 \), serving as the baseline; \textbf{DRCFR B} trains the MT-DRCFR using only the latest available dataset \( D_k \), and thus lacks generalization; \textbf{DRCFR C} does not update the model \( g_{\theta_0}^t(x) \), sacrificing real-time adaptability. 

For the online dataset, we simulate a situation where the exact time of drift occurrence is unknown, but we assume that drift emerges gradually over time. To predict the test dataset for each time period \( k \), where \( k=1,2,\cdots,6\), we again apply ICE-PKD and three comparison strategies. In the incremental updating of \textbf{ICE-PKD}, we begin by selecting an initial model \( g_{\theta_0}^t(x) \) that achieves the best performance on the initially available records and then update the model incrementally with \( D_k \). \textbf{DRCFR A} trains the DR-CFR using the records from the past 9 weeks (including \( D_k \)), serving as the baseline. \textbf{DRCFR B} trains the MT-DRCFR using only the latest available dataset \( D_k \). \textbf{DRCFR C} does not update the model \( g_{\theta_0}^t(x) \). Table \ref{tab:strategy_comparison} below presents a comparative analysis of various strategies, focusing on key aspects such as the use of the latest data, data volume, and whether incremental updates are applied. 

Throughout the experiment, all settings remain consistent, except for the configuration of ICE-PKD, which uses a smaller learning rate and fewer training epochs. Specifically, for the 2-dimensional synthetic dataset, the neural network designed for learning disentangled representations has a hidden layer width of 20 and a depth of 2. The multi-task learning architecture consists of hidden layers with sizes of [10, 20, 10, 20]. The network for the re-weighting function has a hidden layer width of 20 and a depth of 1. The hidden layers for reconstructing the decision rules for treatment assignment have a width of 20 and a depth of 1. The ReLU activation function is applied to these hidden layers, with batch normalization between all adjacent layers. Additionally, L2 regularization with a weight coefficient of 0.01 is applied. The learning rate is set to $1\times10^{-3}$ for non-incremental models and $1\times10^{-4}$ for ICE-PKD. Training epochs are set to 20 for non-incremental models and 10 for ICE-PKD. Additionally, the corrector \( h_{\theta_c} \) in ICE-PKD has a hidden layer width of 20, a depth of 2, Xavier initialization, L2 regularization with strength 0.01, and the output layer uses the tanh activation function. For the online dataset, discrete features, such as dates, are first processed into embedding vectors of dimensionality 10, while continuous features are standardized. The neural network used for learning disentangled representations has a hidden layer width of 128 and a depth of 4. The multi-task learning architecture consists of hidden layers with sizes of [64, 32, 32, 16, 16, 8, 8]. The width of other hidden layers increases from 20 to 128, and the depth of the corrector \( h_{\theta_c} \) is increased from 2 to 4.

\begin{table}
	\caption{Comparative Analysis of Various Strategies}
	\centering
	\begin{tabular}{lcccc}
		\toprule
		\multicolumn{1}{c}{\textbf{Strategy}} & \multicolumn{1}{c}{\textbf{Use of Latest Data}} & \multicolumn{1}{c}{\textbf{Data volume}} & \multicolumn{1}{c}{\textbf{Incremental Updates}} \\
		\midrule
		DRCFR A & Yes & $100,000$  & No \\
		DRCFR B & Yes & $14,000$  & No \\
		DRCFR C & No & $100,000$  & No \\
		ICE-PKD & Yes & $100,000+k\times14,000$  & Yes \\
		\bottomrule
	\end{tabular}
	\label{tab:strategy_comparison}
\end{table}

\subsection{Evaluation Metrics}
In this study, we adopt three commonly used evaluation metrics:  the Average Treatment Effect Error (ATE Error), the Precision in Estimation of Heterogeneous Effect (PEHE) \citep{hill2011bayesian} and QINI Coefficient \citep{radcliffe2007using}. The specific formulas and principles are as follows:

\paragraph{ATE Error.}
ATE Error quantifies the difference between the estimated and true average treatment effects for the treatment group. It helps evaluate the accuracy of the model in predicting the overall treatment effect. In the case with multiple treatments,  the ATE Error is calculated as the average across all treatment groups. The formula is as follows: 
\begin{equation}
   \epsilon_{ATE} = \frac{1}{ n_t}\sum_{t=1}^{n_t}|\hat{\text{ATE}}_t - \text{ATE}_t| 
\end{equation} 

where \( \hat{\text{ATE}}_t\) is the estimated ATE for treatment group \( t \), \( \text{ATE}_t \) is the true ATE for treatment group \( t \), and \( N_t \)
 is the total number of treatment groups.
 
\paragraph{PEHE.}
PEHE evaluates the model's accuracy in predicting heterogeneous treatment effects across the entire population, and it is specifically applied to synthetic datasets. This metric is computed as the square root of the average squared differences between the predicted and true treatment effects, weighted by the population size. The formula of PEHE is: 
\begin{equation}
   \epsilon_{PEHE} = \frac{1}{N \cdot n_t}\sum_{i=1}^{N}\sum_{t=1}^{n_t}{(\hat{\tau}_i^t - \tau_i^t)}^2
\end{equation}

where \( \hat{\tau}_i^t \) is the predicted treatment effect for individual \( i \) in treatment group \( t \), \( \tau_i^t \) is the true treatment effect for individual \( i \) in treatment group \( t \), \( N \) is the total number of individuals, and \( n_t \) is the number of treatment groups.

\paragraph{QINI Coefficient.}

QINI Coefficient is a metric used to evaluate the ranking performance of uplift estimation. It measures the difference in rewards between the treatment group and the control group on a per-segment basis, after sorting the samples by their estimated uplift. To extend its applicability to multi-treatment scenarios, we employ the average QINI Coefficient as a measure of estimation performance. The QINI Coefficient is computed as the area under the QINI Curve. Sort all the quintuples from the treatment group and control group in descending order of estimated individual treatment effect. Denote the top k samples in this sorted list that belong to the treatment group (or control group) by \(Trt(k)\)(or \(Ctr(k)\). QINI Curve could be plotted  after calculating the increment reward \(\Delta Y^{r}(k\) for each point \(1 \leq k \leq N\) by the following formula:

\begin{equation}
   \Delta Reward(k)=\sum_{i \in Trt(k)}  reward_{i}-\frac{|Trt(k)|\sum_{i \in Ctr(k)}  reward_{i}}{|{Ctr(k)}|}
\end{equation}

\subsection{A Proposed Simulation Metric}

Previous evaluation methods have primarily focused on assessing the performance of model estimates in single-treatment scenarios.(modify on-off gap) However, in actual production environments, there is a need for metrics that more accurately reflect the overall performance of online strategies. To address this, we introduce a simulation method, RAS-AUCC (Area Under Cost Curve for Resource Allocation Simulation), which leverages randomized controlled trial(RCT) data to simulate the resource allocation based on model estimation. In addition, this approach makes it possible to simulate the online performance of our generated datasets.

\paragraph{Cost Curve for Resource Allocation Simulation.} Divide all samples into two sets, strategy sets \(Stg\) and control sets \(Ctr\). \(Stg\) includes all treated samples in the trial, while \(Ctr\) includes all samples of the control group in the trial. Apply a certain resource allocation strategy to both sets of samples under a set of budgets \(b\). Retain all samples that have received a treatment in the resource allocation strategy.

Use \(Stg(b)\)(or \(Ctr(b)\)) to denote samples retained under the strategy with budget b in set \(Stg\)(or \(Ctr\)). Similar to the QINI Curve, the incremental reward  \(\Delta Reward(b)\) and incremental cost  \(\Delta Cost(b)\) could be calculated by following formulas:
\begin{equation}
\Delta Cost(b)=(|Stg(b)|+|Ctr(b)|)\left(\frac{\sum_{i \in Stg(b)} \alpha_{i} \beta_{i} cost_i}{|Stg(b)|}-\frac{\sum_{i \in Ctr(b)} cost_{i}}{|Ctr(b)|}\right)
\end{equation}
\begin{equation}
\Delta Reward(b)=(|Stg(b)|+|Ctr(b)|)\left(\frac{\sum_{i \in Stg(b)} \alpha_{i} \beta_{i} reward_i}{|Stg(b)|}-\frac{\sum_{i \in Ctr(b)} reward_{i}}{|Ctr(b)|}\right)
\end{equation}
\begin{equation}
\alpha_{i} = N/N_{t^{rct}_{i}}
\end{equation}
\begin{equation}
\beta_{i} = \begin{cases}
 1 & \text{ if } t^{rct}_{i}=t^{stg}_{i} \\
 0 & \text{ if } t^{rct}_{i}\neq t^{stg}_{i}
\end{cases}
\end{equation}
Here \(t^{rct}_{i}\) denotes the real treatment of sample \(i\), while \(t^{stg}_{i}\) denotes the allocated treatment of sample \(i\) in the strategy. Take the tuple \((\Delta Cost(b),\Delta Reward(b))\) as the coordinates, then the cost curve for simulation is obtained.

\paragraph{Area Under Cost Curve for Resource Allocation Simulation(RAS-AUCC).}
As shown in Figure \ref{fig:RAS-AUCC}, the area under this cost curve \(A_L\) is the proposed simulation metric, and the area under straight line \(A_L\) is used to normalize it. Therefore,RAS-AUCC is defined as \((A_S - A_L)/A_L\).

\begin{figure}
    \centering
    \includegraphics[height=6cm]{ras-aucc.pdf} 
    \caption{RAS-AUCC}
    \label{fig:RAS-AUCC}
\end{figure}

In our application scenario, the resource allocation DRCFR can be simplified to marginal ROI ranking. Therefore, we use the marginal ROI ranking strategy to calculate RAS-AUCC here.


\subsection{Evaluation Framework for Continual Causal Effects Estimation}
In the estimation of continual causal effects, various evaluation metrics are employed, such as ATE Error and RAS-AUCC, particularly for assessing multiple time periods. Therefore, it is crucial to establish a comprehensive and robust assessment framework for this context. A common approach is to compare the average difference of each metric across time periods. However, this method has its limitations, as it is highly sensitive to extreme values. Specifically, a substantial increase or decrease in a certain time period can distort the observed effects at other time periods. To address this challenge, from the perspective of stability and significance, we propose the use of two stability indicators, in addition to an average indicator, to jointly evaluate the model's performance.

\paragraph{PRIO-10.}
The Percentage of Relative Improvement Over 10\% (PRIO-10) measures the proportion of cases where the improvement of the model exceeds 10\%. This indicator helps assess the overall performance gain relative to the baseline. Specifically, given the Baseline \( M_{\text{baseline}} \), for any model \( A \), and for any evaluation metric \( E \) that benefits from larger values (such as QINI and RAS-AUCC), the improvement \citep{zhong2022descn} is calculated as:
\begin{equation}
    Impr_k(A)=\frac{E_k(A)-E_k(M_{\text{baseline}})}{|E_k(M_{\text{baseline}})|} \times 100 \%, \quad k=1,2,\cdots,n_k
\end{equation}

where \(k\) represents the different time periods. The PRIO-10 for method A is then calculated as:
\begin{equation}
    \text{PRIO-10}(A)=\frac{1}{n_k}\sum_{k=1}^{n_k}\mathbf{1}_{\{Impr_k(A)>10\%\}}(A) \times 100\%
\end{equation}

In contrast, for any evaluation metric that improves with smaller values, such as ATE Error and RMSE of PEHE, the improvement is calculated by multiplying the result by \( -1 \).

\paragraph{PRDU-5.}
The Percentage of Relative Deterioration Under 5\% (PRDU-5) measures the proportion of cases where the deterioration in performance is under 5\%. This metric is used to assess how well the model performs in avoiding significant declines. Similar to PRIO-10, given the Baseline \( M_{\text{baseline}} \), for any model \( A \), and for any evaluation metric \( E \) that benefits from larger values, the PRDU-5 is calculated as follows:
\begin{equation}
        \text{PRDU-5}(A) = \frac{1}{n_k} \sum_{k=1}^{n_k} \mathbf{1}_{\{ -Impr_k(A) < 5\% \}} \times 100\%
\end{equation}

\paragraph{AD.}
The Average Difference (AD) assesses the model's overall performance across all time periods by calculating the average of the metric differences between the model and the baseline. Specifically, given the Baseline \( M_{\text{baseline}} \), for any model \( A \), and for any evaluation metric \( E \), the AD is calculated as:
\begin{equation}
    \text{AD}(A)=\frac{1}{n_k} \sum_{k=1}^{n_k} [E_k(A)-E_k(M_{\text{baseline}})]
\end{equation}

\section{Experiment Results}
This section presents the results of our experiments, offering a comparative analysis of various strategies using different evaluation metrics. Additionally, we provide an explanation of each module's contribution.

\subsection{Performance Comparison}
We evaluate the effectiveness of ICE-PKD by comparing it against other strategies on both synthetic and online datasets, as shown in Table \ref{tab:comparison}. The experimental setup is detailed in Section \ref{section:experimental setting}. Key insights from the results are summarized below.

Compared to the baseline, DRCFR A, ICE-PKD consistently achieves superior performance. Specifically, ICE-PKD achieves the largest reduction in error class metrics  \( \epsilon_{ATE} \) and \( \epsilon_{PEHE} \), as well as the most significant improvement in order metrics QINI and RAS-AUCC. Furthermore, ICE-PKD outperforms all other strategies across all indicators for PRIO-10 and PRDU-5, indicating that its performance is not influenced by extreme values. This suggests that ICE-PKD is robust and effective. 

On the other hand, DRCFR B, which is trained solely on the most recent dataset \( D_k \), exhibits lower performance in order metrics. On the 2-dimensional synthetic dataset, it is outperformed by both DRCFR C and ICE-PKD in terms of \( \epsilon_{PEHE} \). Although DRCFR B performs better than DRCFR C in AD for RAS-AUCC, it significantly lags behind in PRIO-10 and PRDU-5, which is  undesirable. On the 10-dimensional synthetic dataset, it performs worse than DRCFR C in AD for RAS-AUCC, further highlighting its unreliability. On the online dataset, DRCFR B's performance is even worse, significantly trailing the baseline in both QINI and RAS-AUCC. These results suggest that DRCFR B lacks generalization and may overfit when working with smaller datasets. 

DRCFR C, which does not update the initial model \(g_{\theta_0}^t(x)\), shows poorer performance across the error metrics. Notably, it performs the worst in \( \epsilon_{ATE} \), being the only strategy significantly worse than the baseline for both the 2-dimensional synthetic dataset and the online dataset. Although DRCFR C performs well on most AD indicators, its stability indicators (PRIO-10 and PRDU-5) are generally the worst, suggesting that it is not a reliable choice. The poor performance can be attributed to the model's lack of real-time adaptability, particularly in the presence of covariate shift and concept drift.

To further illustrate these findings, we visualize the comparison results for the 2-dimensional synthetic dataset in Figure \ref{fig:comparison}. The vertical axis represents the difference between each strategy's metrics and the baseline's across different time periods \( k \). ICE-PKD (represented by the purple line with circular marker points) consistently performs best, located at the bottom of the subplots for \( \epsilon_{ATE} \) and \( \epsilon_{PEHE} \), and at the top of the subplots for QINI and RAS-AUCC. In contrast, DRCFR B (yellow line with triangle markers) shows significant fluctuations due to the smaller training set. DRCFR C (green line with square markers) performs poorly, particularly in \( \epsilon_{ATE} \) and \( \epsilon_{PEHE} \), due to its lack of real-time adaptability. These visual observations closely align with the analytical results discussed above. 

In conclusion, ICE-PKD outperforms all other strategies across both datasets, demonstrating its robustness, adaptability, and effectiveness in addressing covariate shift and concept drift while maintaining stable and reliable performance over time.

\begin{table}
	\caption{Performance comparison of different strategies on synthetic and online datasets}
	\centering
        \resizebox{\textwidth}{!}{
	\begin{tabular}{clllllllllllll}
		\toprule
		& & \multicolumn{3}{c}{$\epsilon_{ATE}$} & \multicolumn{3}{c}{$\epsilon_{PEHE}$} & \multicolumn{3}{c}{QINI} & \multicolumn{3}{c}{RAS-AUCC}\\
		\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
            & strategy & \small{PRIO-10} & \small{PRDU-5} & \small{AD} & \small{PRIO-10} & \small{PRDU-5} & \small{AD} & \small{PRIO-10} & \small{PRDU-5} & \small{AD} & \small{PRIO-10} & \small{PRDU-5} & \small{AD}\\
            \midrule
            \multirow{3}{*}[0pt]{\parbox[c][3\baselineskip]{1cm}{\centering synthetic \newline  dataset \newline 2d}}
                & DRCFR A & - & - & 0 & - & - & 0 & - & - & 0 & - & - & 0\\
                & DRCFR B & 83.3\% & 83.3\% & -0.0065 & 50\% & 66.7\% & 0.0028 & 83.3\% & 83.3\% & 0.0286 & 66.7\% & 66.7\% & 0.0566\\
                & DRCFR C & 33.3\% & 50\% & 0.0032 & 50\% & 66.7\% & -0.0017 & 66.7\% & 66.7\% & 0.0233 & 100\% & 100\% & 0.0457\\
                & ICE-PKD & 100\% & 100\% & -0.0313 & 100\% & 100\% & -0.0195 & 100\% & 100\% & 0.0418 & 100\% & 100\% & 0.0669\\
            \midrule
            \multirow{3}{*}[0pt]{\parbox[c][3\baselineskip]{1cm}{\centering synthetic \newline  dataset \newline 10d}}
                & DRCFR A & - & - & 0 & - & - & 0 & - & - & 0 & - & - & 0\\
                & DRCFR B & 16.7\% & 33.3\% & 0.0073 & 33.3\% & 66.7\% & -0.0164 & 16.7\% & 33.3\% & -0.0019 & 66.7\% & 66.7\% & 0.0161\\
                & DRCFR C & 0\% & 0\% & 0.0154 & 33.3\% & 33.3\% & -0.0104 & 16.7\% & 16.7\% & -0.0155 & 66.7\% & 66.7\% & 0.0540\\
                & ICE-PKD & 83.3\% & 100\% & -0.0177 & 100\% & 100\% & -0.0276 & 100\% & 100\% & 0.0112 & 66.7\% & 100\% & 0.0699\\
            \midrule
            \multirow{3}{*}{\parbox[c]{1cm}{online\\ dataset}} 
                & DRCFR A & - & - & 0 & - & - & - & - & - & 0 & - & - & 0\\
                & DRCFR B & 50\% & 50\% & -0.0002 & - & - & - & 33.3\% & 33.3\% & -0.0289 & 50\% & 50\% & -0.0097\\
                & DRCFR C & 33.3\% & 33.3\% & 0.0039 & - & - & - & 66.7\% & 83.3\% & 0.0213 & 83.3\% & 100\% & 0.0789\\
                & ICE-PKD & 66.7\% & 100\% & -0.0023 & - & - & - & 83.3\% & 83.3\% & 0.0273 & 83.3\% & 100\% & 0.0495\\
		\bottomrule
	\end{tabular}}
	\label{tab:comparison}
\end{table}

\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.24\textwidth} % 控制子图宽度
        \centering
        \includegraphics[width=\textwidth]{ate.pdf}
    \end{minipage}\hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pehe.pdf}
    \end{minipage}\hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{QINI.pdf}
    \end{minipage}\hfill
    \begin{minipage}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{mtaucc.pdf}
    \end{minipage}
    \caption{Comparison of performance metrics across different strategies}
    \label{fig:comparison}
\end{figure}

\subsection{Ablation Experiment}
To further evaluate the contribution of each component in ICE-PKD, we conducted an ablation experiment on the synthetic dataset. In this experiment, we systematically removed key components of the model to assess their impact on performance. The results are presented in Table \ref{tab:ablation}.

We define three variants of ICE-PKD by removing the following components:

\textbf{w/o PT:} ICE-PKD without the proxy teacher for knowledge distillation.

\textbf{w/o RM:} ICE-PKD without the replay mechanism.

\textbf{w/o KD} ICE-PKD without the knowledge distillation process.

For each variant, the experimental setup remains consistent with the one described for ICE-PKD in Section \ref{section:experimental setting}. From the results in Table \ref{tab:ablation}, we can draw the following key insights:

\textbf{Impact of Proxy Teacher (PT):} Removing the proxy teacher for knowledge distillation (w/o PT) leads to a noticeable decline in overall performance across all metrics. Specifically, \( \epsilon_{ATE} \) and \( \epsilon_{PEHE} \) show increased error values, with the AD for these metrics worsening from -0.0313 to -0.0270 and from -0.0195 to -0.0171, respectively. Additionally, both QINI and RAS-AUCC exhibit decreased values, with the AD dropping from 0.0418 to 0.0397 and 0.0669 to 0.0634, respectively. These results emphasize the critical role of the proxy teacher in knowledge distillation, as it helps improve the overall performance of ICE-PKD by preventing the model from blindly mimicking the teacher, especially in the presence of concept drift.

\textbf{Impact of Replay Mechanism (RM):} Removing the replay mechanism (w/o RM) results in the most significant decrease in performance, particularly for RAS-AUCC. Specifically, the PRIO-10 drops from 100\% to 83.3\%, and the AD decreases from 0.0669 to 0.0434. These results highlight the importance of preserving previous knowledge through the replayed dataset. Since neural network models tend to perform poorly on out-of-distribution data, relying solely on knowledge distillation with the latest available data can steer the model in the wrong direction when faced with covariate shift.

\textbf{Impact of Knowledge Distillation (KD):} Excluding the knowledge distillation process (w/o KD) has significant negative effects on stability indicators. Specifically, PRIO-10 for \( \epsilon_{ATE} \) and \( \epsilon_{PEHE} \) decreases to 83.3\% and 66.7\%, respectively, while PRDU-5 for \( \epsilon_{ATE} \) also drops to 83.3\%. These results demonstrate the crucial role of knowledge distillation in maintaining stable and accurate predictions over time.

\textbf{Full Model (ICE-PKD):} The full ICE-PKD model consistently outperforms its ablated variants across all metrics, achieving the lowest average error metrics, the highest average order metrics, and the highest stability indicators. For instance, ICE-PKD achieves 100\% in both PRIO-10 and PRDU-5 for \( \epsilon_{PEHE} \) and RAS-AUCC, along with the lowest AD values for \( \epsilon_{PEHE} \) and the highest for RAS-AUCC. These results confirm the effectiveness of integrating all components in the proposed model.

The ablation experiment highlights the critical contributions of proxy teacher, replay mechanism, and knowledge distillation to the overall performance of ICE-PKD. The results demonstrate that these components collectively enhance the model's robustness, stability, and accuracy, further validating the design of ICE-PKD.

\begin{table}
	\caption{Ablation study on synthetic dataset}
	\centering
        \resizebox{\textwidth}{!}{
	\begin{tabular}{clllllllllllll}
		\toprule
		& & \multicolumn{3}{c}{$\epsilon_{ATE}$} & \multicolumn{3}{c}{$\epsilon_{PEHE}$} & \multicolumn{3}{c}{QINI} & \multicolumn{3}{c}{RAS-AUCC}\\
		\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
            & strategy & \small{PRIO-10} & \small{PRDU-5} & \small{AD} & \small{PRIO-10} & \small{PRDU-5} & \small{AD} & \small{PRIO-10} & \small{PRDU-5} & \small{AD} & \small{PRIO-10} & \small{PRDU-5} & \small{AD}\\
            \midrule
            \multirow{3}{*}{\parbox[c]{1cm}{synthetic\\ dataset}} 
                & ICE-PKD & 100\% & 100\% & -0.0313 & 100\% & 100\% & -0.0195 & 100\% & 100\% & 0.0418 & 100\% & 100\% & 0.0669\\
                & w/o PT & 83.3\% & 100\% & -0.0270 & 83.3\% & 100\% & -0.0171 & 100\% & 100\% & 0.0397 & 100\% & 100\% & 0.0634\\
                & w/o RM & 100\% & 100\% & -0.0257 & 83.3\% & 100\% & -000169 & 100\% & 100\% & 0.0421 & 83.3\% & 100\% & 0.0434\\
                & w/o KD & 83.3\% & 83.3\% & -0.0271 & 66.7\% & 100\% & -0.0170 & 100\% & 100\% & 0.0407 & 100\% & 100\% & 0.0637\\
		\bottomrule
	\end{tabular}}
	\label{tab:ablation}
\end{table}

\subsection{Citations}
Citations use \verb+natbib+. The documentation may be found at
\begin{center}
	\url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}

\subsection{Figures}
\lipsum[10]
See Figure \ref{fig:fig1}. Here is how you add footnotes. \footnote{Sample of the first footnote.}
\lipsum[11]

\begin{figure}
	\centering
	\fbox{\rule[-.5cm]{4cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
	\caption{Sample figure caption.}
	\label{fig:fig1}
\end{figure}

\subsection{Tables}
See awesome Table~\ref{tab:table}.

The documentation for \verb+booktabs+ (`Publication quality tables in LaTeX') is available from:
\begin{center}
	\url{https://www.ctan.org/pkg/booktabs}
\end{center}


\begin{table}
	\caption{Sample table title}
	\centering
	\begin{tabular}{lll}
		\toprule
		\multicolumn{2}{c}{Part}                   \\
		\cmidrule(r){1-2}
		Name     & Description     & Size ($\mu$m) \\
		\midrule
		Dendrite & Input terminal  & $\sim$100     \\
		Axon     & Output terminal & $\sim$10      \\
		Soma     & Cell body       & up to $10^6$  \\
		\bottomrule
	\end{tabular}
	\label{tab:table}
\end{table}

\subsection{Lists}
\begin{itemize}
	\item Lorem ipsum dolor sit amet
	\item consectetur adipiscing elit.
	\item Aliquam dignissim blandit est, in dictum tortor gravida eget. In ac rutrum magna.
\end{itemize}

\section{Conclusion}
In this paper, we propose the ICE-PKD framework to address the challenges of causal effect estimation in dynamic environments, particularly in marketing, where covariate shift and concept drift are common. Our approach extends the DR-CFR framework to handle multiple treatments and introduces a novel method for continual causal effect estimation. By incorporating key components such as initial model selection, replay mechanism and proxy teacher knowledge distillation, ICE-PKD provides a robust and adaptable solution for estimating continual causal effects in the presence of covariate shift and concept drift. 

The experimental results demonstrate that ICE-PKD consistently outperforms other strategies across both synthetic and real-world online datasets. Our method not only addresses covariate shift and concept drift effectively but also ensures stable and reliable performance over time. Furthermore, ablation experiments highlight the crucial roles played by the proxy teacher, reply mechanism, and knowledge distillation in enhancing the model's performance and robustness.

Overall, ICE-PKD represents a significant advancement in the field of continual causal effect estimation, providing a more effective and robust approach for dynamic marketing environments. Several promising avenues for future research include exploring uplift models that are more suitable for estimating continuous causal effects and delving into more advanced incremental learning methods, such as enhanced knowledge distillation techniques, improved replay mechanisms, and other specialized structures. 

\bibliographystyle{unsrtnat}
\bibliography{references} 

\end{document}

